LAS-AT: Adversarial Training with Learnable Attack Strategy

Adversarial training (AT) is always formulated as a minimax problem, of which the performance depends on the inner optimization that involves the generation of adversarial examples (AEs). Most previous methods adopt Projected Gradient Decent (PGD) with manually specifying attack parameters for AE generation. A combination of the attack parameters can be referred to as an attack strategy. Several works have revealed that using a fixed attack strategy to generate AEs during the whole training phase limits the model robustness and propose to exploit different attack strategies at different training stages to improve robustness. But those multi-stage hand-crafted attack strategies need much domain expertise, and the robustness improvement is limited. In this paper, we propose a novel framework for adversarial training by introducing the concept of "learnable attack strategy", dubbed LAS-AT, which learns to automatically produce attack strategies to improve the model robustness. Our framework is composed of a target network that uses AEs for training to improve robustness and a strategy network that produces attack strategies to control the AE generation. Experimental evaluations on three benchmark databases demonstrate the superiority of the proposed method. The code is released at https://github.com/jiaxiaojunQAQ/LAS-AT.

==> figtex/fig_policy.tex <==
\begin{figure}[t]
\begin{center}
   \includegraphics[width=1.0\linewidth]{image/Fig2_v2.pdf}
\end{center}
\vspace{-3mm}
   \caption{The overview of the strategy network. 
   The outputs are a set of attack parameters for generating adversarial examples. Each attack parameter is encoded by a one-hot vector. }
\label{fig:santan2}
\vspace{-3mm}
\end{figure}

%The  basic  architecture  of  the  policy  network  for  generating the corresponding adversarial operations.  Each operation parameter corresponds to the output of the policy network.  And these outputs share information through the shared network and work together with each other to produce the corresponding adversarial attack policy.

==> figtex/fig_reward.tex <==
\begin{figure*}[t]
\begin{center}
   \includegraphics[width=0.95\linewidth]{latex/image/Fig4.pdf}
\end{center}
\vspace{-3mm}
   \caption{The reward curve during adversarial training when the target models are fixed. (a) The target network is randomly initialized. (b) The target network is trained with benign images. (c) The target network is trained with adversarial examples.}
\label{fig:converge}
\end{figure*}

==> table/tb_Comparison_AT_cifar10.tex <==
\begin{table}[t]
\centering

\caption{Comparisons with on most advanced adversarial training methods on the CIFAR10 database. 
Numbers represent percentage. Number with underline indicates the best. }
\vspace{-3mm}
 \label{tb:Comparison_AT_cifar10}
 \scalebox{0.85}{
\begin{tabular}{c|c|c|c}
\hline
Target network                   & Method               & Clean          & AA             \\ \hline \hline
\multirow{2}{*}{WideResNet34-10} & Trades-AWP           & \textbf{85.36} & 56.17          \\ \cline{2-4} 
                                 & LAS-Trades-AWP(ours) & 84.98          & \textbf{56.28} \\ \hline \hline
\multirow{2}{*}{WideResNet70-16} & ULAT                 & 85.29          & 57.20          \\ \cline{2-4} 
                                 & LAS-Trades-AWP(ours) & \textbf{85.66} & \textbf{57.61} \\ \hline
\end{tabular}

}
\vspace{-3mm}
\end{table}

==> table/tb_Comparison_AT_cifar100.tex <==
\begin{table}[t]
\centering

\caption{Comparisons with on most advanced adversarial training methods on the CIFAR100 database. 
Numbers represent percentage. Number with underline indicates the best. }
\vspace{-3mm}
 \label{tb:Comparison_AT_cifar10}
 \scalebox{0.9}{
\begin{tabular}{c|c|c|c}
\hline
Target network                   & Method        & Clean          & AA             \\ \hline \hline
\multirow{3}{*}{WideResNet34-10} & AWP-AT        & 60.38          & 28.86          \\ \cline{2-4} 
                                 & LBGAT         & 60.64          & 29.33          \\ \cline{2-4} 
                                 & LAS-AWP(ours) & \textbf{64.89} & \textbf{30.77} \\ \hline \hline
\multirow{2}{*}{WideResNet34-20} & LBGAT         & 62.55          & 30.20          \\ \cline{2-4} 
                                 & LAS-AWP(ours) & \textbf{67.31} & \textbf{31.92} \\ \hline
\end{tabular}

}
\vspace{-3mm}
\end{table}

==> table/tb_Comparison_AT_cifar10_v2.tex <==
\begin{table}[t]
\centering

\caption{Comparisons with on most advanced adversarial training methods on the CIFAR10 database. 
Numbers represent percentage. Number with underline indicates the best. }
\vspace{-3mm}
 \label{tb:Comparison_AT_cifar10}
 \scalebox{0.85}{
\begin{tabular}{c|c|c|c}
\hline
Target network                   & Method               & Clean          & AA             \\ \hline \hline

\multirow{2}{*}{WideResNet70-16} & ULAT                 & 85.29          & 57.20          \\ \cline{2-4} 
                                 & LAS-AWP(ours) & \textbf{85.66} & \textbf{57.61} \\ \hline
\end{tabular}

}
\vspace{-3mm}
\end{table}

==> table/tb_ablation.tex <==
\begin{table}[t]
\centering

\caption{Ablation study results on the CIFAR10 database. Numbers in table represent percentage. }
\vspace{2mm}
 \label{table:table0}
\begin{tabular}{C{1.9cm}|C{1.2cm}|C{1.3cm}|C{1.8cm}}
\hline
Method & $R_{1}$    & $R_{1}+R_{2}$ & $R_{1}+R_{2}-b$ \\ \hline \hline
Clean  & \textbf{90.39} & 80.88 & 82.84   \\ \hline\hline
PGD-10 & 48.5  & 54.04 & \textbf{54.10}  \\ 
APGD  & 27.70 & 51.20 & \textbf{51.60}   \\ 
APGD-T & 34.79 & \textbf{53.50} & 52.10   \\ 
FAB    & 64.30 & 70.90 & \textbf{72.40}   \\ 
SQUARE & \textbf{79.60} & 73.90 & 74.90   \\ 
AA     & 23.00 & 41.80 & \textbf{42.40}   \\ \hline
Mean   & 46.32 & 57.56 & \textbf{57.92}   \\ \hline
\end{tabular}
\end{table}

==> table/tb_ablation_v2.tex <==
\begin{table}[t]
\centering

\caption{Ablation study results on the CIFAR10 database. Numbers in table represent percentage. }
\vspace{2mm}
 \label{table:table0}
\begin{tabular}{CCCC|C}
\hline
Method & $R_{1}$    & $R_{2}$    & $R_{1}+R_{2}$ & $R_{1}+R_{2}-b $       \\ \hline
clean  & 81.83 & 81.67 & 81.32 & \textbf{82.05} \\ \hline
PGD-10 & 53.88 & 54.03 & 53.83 & \textbf{54.23} \\ \hline
APGD   & 52.43 & 52.53 & 52.40 & \textbf{53.03} \\ \hline
APGD-T & 49.25 & 49.44 & 49.29 & \textbf{50.08} \\ \hline
FAB    & 49.68 & 49.82 & 49.65 & \textbf{50.38} \\ \hline
SQUARE & 55.64 & 55.68 & 55.74 & \textbf{56.13} \\ \hline
AA     & 49.26 & 49.44 & 49.21 & \textbf{50.07} \\ \hline
\end{tabular}
\end{table}

==> table/tb_ablation_v3.tex <==
\begin{table}[t]
\centering

\caption{Ablation study results on the CIFAR10 database. Numbers in table represent percentage. }
\vspace{-3mm}
 \label{table:table0}
\begin{tabular}{c|ccc}
\hline
Method & $L_0$  & $L_0$ \& $L_1$ & $L_0$ \& $L_1$ \& $L_2$       \\ \hline\hline
clean  & 81.83 & 81.54 & \textbf{82.05} \\ \hline\hline
PGD-10 & 53.88 & 54.08 & \textbf{54.23} \\ 
APGD   & 52.43 & 52.68 & \textbf{53.03} \\ 
APGD-T & 49.25 & 49.55 & \textbf{50.08} \\ 
FAB    & 49.68 & 49.90 & \textbf{50.38} \\ 
SQUARE & 55.64 & 55.78 & \textbf{56.13} \\ 
AA     & 49.26 & 49.54 & \textbf{50.07} \\ \hline
\end{tabular}
\end{table}

==> table/tb_ablation_v4.tex <==
\begin{table}[t]
\centering

\caption{Ablation study results on the CIFAR10 database. Numbers in table represent percentage. }
\vspace{-3mm}
 \label{table:table0}
  \scalebox{0.89}{
\begin{tabular}{c|cccc}
\hline
Method & $L_0$ & $L_0$ \& $L_1$ & $L_0$ \& $L_2$ & $L_0$ \& $L_1$ \& $L_2$ \\ \hline \hline
clean  & 81.83 & 81.54          & 81.90          & \textbf{82.3}          \\ \hline \hline
PGD-10 & 53.88 & 54.08          & 53.89          & \textbf{54.29}          \\ 
APGD   & 52.43 & 52.68          & 52.30          & \textbf{52.91}          \\ 
APGD-T & 49.25 & 49.55          & 49.30          & \textbf{50.08}          \\ 
FAB    & 49.68 & 49.90          & 49.71          & \textbf{50.38}          \\ 
SQUARE & 55.64 & 55.78          & 55.58          & \textbf{56.13}          \\ 
AA     & 49.26 & 49.54          & 49.30          & \textbf{49.89}          \\ \hline
\end{tabular}
}
\vspace{-3mm}
\end{table}

==> table/tb_cifar10.tex <==
\begin{table*}[t]
\centering

\caption{Comparisons with state-of-the-art methods on the CIFAR10 database. 
Numbers in table represent percentage. $\uparrow$ and $\downarrow$ indicate performance change after plugging in our RLAT compared to the corresponding base model. Accuracy number in bold indicates the best. }
\vspace{2mm}
 \label{tb:cifar10}
 \scalebox{0.82}{
\begin{tabular}{c|c|cccccc|c}
\hline
Method        & Clean          & PGD-10         & APGD           & APGD-T         & FAB            & SQUARE         & AA             & Mean           \\ \hline \hline


Standard     & 94.72          & 0.0            & 1.80           & 1.40           & 63.00          & 64.70          & 0.0            & 21.82        \\ \hline\hline


SAT~\cite{madry2017towards}          & {84.50}  & 50.65          & 45.20          & 46.10          & 67.20          & 73.30          & 38.60          & 53.51          \\


Trades~\cite{zhang2019theoretically}       & {82.20}          & 52.68          & 48.90          & 48.00          & 71.70          & {73.50}          & 39.82          & 55.77          \\

Avmixup~\cite{lee2020adversarial}      & 87.83          & 45.21          & 36.80          & 42.60          & 68.30          & \textbf{79.00}          & 18.30          & 48.37          \\\hline


RLAT-SAT     & 82.84 $\downarrow$  1.66   & {54.1} $\uparrow$ \textbf {3.45}  & {51.60} $\uparrow$ \textbf {6.40} & {52.10} $\uparrow$ \textbf {6.00} & {72.40}  $\uparrow$ \textbf {5.20} & {74.90}  $\uparrow$ \textbf {1.60}  & {42.40} $\uparrow$ \textbf {3.80}  & {57.92} $\uparrow$ \textbf {4.41} \\ 


RLAT-Trades  & 80.97  $\downarrow$ 1.23         & \textbf{54.23} $\uparrow$ \textbf {1.55} & {51.90} $\uparrow$ \textbf {3.00} & {50.60} $\uparrow$ \textbf {2.60} & {71.80} $\uparrow$ \textbf{0.10}  & 72.90 $\downarrow$ 0.60 & {43.60} $\uparrow$ \textbf  {3.78} & {57.51} $\uparrow$ \textbf {1.74} \\ 


RLAT-Avmixup & \textbf{90.71} $\uparrow$  \textbf{2.88} & {53.66} $\uparrow$ \textbf {8.45} & \textbf{58.40} $\uparrow$ \textbf {21.60} & \textbf{59.20} $\uparrow$ \textbf {16.60}   & \textbf{74.50} $\uparrow$ \textbf {6.20} & \textbf{79.00}  & \textbf{46.88}$\uparrow$ \textbf  {28.58}& \textbf{61.94} $\uparrow$ \textbf {13.57}  \\ \hline
\end{tabular}
}
\end{table*}

==> table/tb_cifar100.tex <==
\begin{table*}[t]
\centering

\caption{Comparisons with state-of-the-art methods on the CIFAR100 database. 
Numbers in table represent percentage. $\uparrow$ and $\downarrow$ indicate performance change after plugging in our RLAT compared to the corresponding base model. Accuracy number in bold indicates the best. }
\vspace{2mm}
 \label{tb:cifar100}
 \scalebox{0.82}{
\begin{tabular}{c|c|cccccc|c}
\hline
Method        & Clean          & PGD-10         & APGD           & APGD-T         & FAB            & SQUARE         & AA             & Mean           \\ \hline \hline
Standard     & 77.95          & 0.02          & 4.30           & 4.70           & 46.00          & 48.10          & 0.0            & 17.18          \\ \hline\hline

SAT~\cite{madry2017towards}         & {58.97} & 26.68          & 28.60          & 32.20          & 47.10          & 48.80          & 19.00          & 33.73          \\

Trades~\cite{zhang2019theoretically}       & 54.56          & 28.34          & 30.30          & 34.30          & 44.80          & 46.20          & {19.80} & 33.96         \\


Avmixup~\cite{lee2020adversarial}       & 65.26          & 28.18          & 29.15          & 31.30          & \textbf{51.20} & \textbf{54.80} & 15.20          & 34.97        \\ \hline

RLAT-SAT     & 58.3  $\downarrow$   0.67      & {29.01} $\uparrow$ \textbf {2.33}& {31.90} $\uparrow$ \textbf {3.30} & {35.00} $\uparrow$ \textbf {2.80} & {48.90} $\uparrow$ \textbf {1.80} & {50.20} $\uparrow$ \textbf  {1.40}& {20.20} $\uparrow$ \textbf {1.20} & {35.87} $\uparrow$ \textbf  {2.14}\\ 

RLAT-Trades  & {58.89} $\uparrow$ \textbf {4.33} & {30.76} $\uparrow$ \textbf {2.42} & {31.60} $\uparrow$ \textbf {1.30}& {35.20} $\uparrow$ \textbf {0.9} & {49.30} $\uparrow$ \textbf {4.50} & {49.60} $\uparrow$ \textbf {3.40} & 18.40  $\downarrow$   1.40       & {35.81} $\uparrow$ \textbf  {1.85}\\

RLAT-Avmixup & \textbf{67.49} $\uparrow$ \textbf {2.23} & \textbf{33.30} $\uparrow$ \textbf {5.13} & \textbf{38.90} $\uparrow$ \textbf  {9.75}& \textbf{41.90} $\uparrow$ \textbf {10.60} & 50.40 $\downarrow$  0.80        & 52.80    $\downarrow$  2.00     & \textbf{24.00} $\uparrow$ \textbf {8.80} & \textbf{40.21} $\uparrow$ \textbf {5.24} \\ \hline
\end{tabular}
}
\end{table*}

==> table/tb_cifar100_v2.tex <==
\begin{table*}[t]
\centering
\footnotesize{
\caption{ The comparison result on CIFAR100. }
 \label{table:table2}
\begin{tabular}{c|c|cccccc|c}
\hline
Method       & Clean          & PGD-10         & APGD           & APGD-T         & FAB            & SQUARE         & AA             & Mean           \\ \hline \hline
Standard     & 77.95          & 0.02          & 4.30           & 4.70           & 46.00          & 48.10          & 0.0            & 17.18          \\ \hline\hline
SAT~\cite{madry2017towards}         & \textbf{58.97} & 26.68          & 28.60          & 32.20          & 47.10          & 48.80          & 19.00          & 33.73          \\
RLAT-PGD     & 58.3  $\downarrow$   0.67      & \textbf{29.01} $\uparrow$ \textbf{2.33}& \textbf{31.90} $\uparrow$ \textbf{3.30} & \textbf{35.00} $\uparrow$ \textbf{2.80} & \textbf{48.90} $\uparrow$ \textbf{1.80} & \textbf{50.20} $\uparrow$  \textbf{1.40}& \textbf{20.20} $\uparrow$ \textbf{1.20} & \textbf{35.87} $\uparrow$  \textbf{2.14}\\ \hline
Trades~\cite{zhang2019theoretically}       & 54.56          & 28.34          & 30.30          & 34.30          & 44.80          & 46.20          & \textbf{19.80} & 33.96         \\
RLAT-Trades  & \textbf{58.89} $\uparrow$ \textbf{4.33} & \textbf{30.76} $\uparrow$ \textbf{2.42} & \textbf{31.60} $\uparrow$ \textbf{1.30}& \textbf{35.20} $\uparrow$ \textbf{0.9} & \textbf{49.30} $\uparrow$ \textbf{4.50} & \textbf{49.60} $\uparrow$ \textbf{3.40} & 18.40  $\downarrow$   1.40       & \textbf{35.81} $\uparrow$  \textbf{1.85}\\ \hline
Avmixup~\cite{lee2020adversarial}       & 65.26          & 28.18          & 29.15          & 31.30          & \textbf{51.20} & \textbf{54.80} & 15.20          & 34.97        \\
RLAT-Avmixup & \textbf{67.49} $\uparrow$ \textbf{2.23} & \textbf{33.30} $\uparrow$ \textbf{5.13} & \textbf{38.90} $\uparrow$  \textbf{9.75}& \textbf{41.90} $\uparrow$ \textbf{10.60} & 50.40 $\downarrow$  0.80        & 52.80    $\downarrow$  2.00     & \textbf{24.00} $\uparrow$ \textbf{8.80} & \textbf{40.21} $\uparrow$ \textbf{5.24} \\ \hline
\end{tabular}
}
\end{table*}

==> table/tb_cifar100_v3.tex <==
\begin{table*}[t]

\centering

\caption{ Comparisons on the CIFAR100 database. 
Numbers represent percentage. Number with underline indicates the best. 
%$\uparrow$ and $\downarrow$ indicate the performance change after the combination with our framework. 
`a $\uparrow$ b' denotes that the accuracy is `a' and the improvement over the corresponding base model is `b'. `$\uparrow$' means `increase' and `$\downarrow$' means `decrease'. 
}
 \label{tb:cifar100}
 
 \vspace{-3mm}
 \scalebox{0.82}{
\begin{tabular}{c|c|cc|ccccc}
\hline
      Target network                    & Method       & Clean          & PGD-10         & APGD           & APGD-T         & FAB            & SQUARE         & AA             \\ \hline \hline
 & PGD-AT ~\cite{rice2020overfitting}     & 56.23          & 29.52          & 28.57          & 24.79          & 24.99          & 30.31          & 24.78          \\ %\cline{2-9} 
                          & Trades~\cite{zhang2019theoretically}       & 56.57          & 28.54          & 27.88          & 23.97          & 24.26          & 28.16          & 23.98          \\ %\cline{2-9} 
                          & AVmixup~\cite{lee2020adversarial}     & 63.81          & 31.62          & 24.91          & 16.03          & 16.77          & 26.08          & 15.23          \\ \cline{2-9} 
       Resnet18  & LAS-PGD-AT   &   {58.15} $\uparrow$ \textbf{1.92} &   {31.97} $\uparrow$ \textbf{2.45} &   \underline{30.94} $\uparrow$ \textbf{2.37} &   \underline{26.52} $\uparrow$ \textbf{1.73} &   \underline{26.75} $\uparrow$ \textbf{1.76} &  \underline {31.52} $\uparrow$ \textbf{1.21} &   \underline{26.50} $\uparrow$ \textbf{1.72}\\ %\cline{2-9} 
              & LAS-Trades  &   {58.09} $\uparrow$ \textbf{1.52} &   {29.88} $\uparrow$ \textbf{1.34} &   {29.22} $\uparrow$ \textbf{1.34}&   {25.21} $\uparrow$ \textbf{1.24} &   {25.42} $\uparrow$ \textbf{1.16} &   {29.62} $\uparrow$ \textbf{1.46}&   {25.21} $\uparrow$ \textbf{1.23} \\ %\cline{2-9} 
              & LAS-AVmixup &   \underline{65.04} $\uparrow$ \textbf{1.23} &   \underline{34.20} $\uparrow$ \textbf{2.58} & 23.75 $\downarrow$ 1.16    &   {17.17} $\uparrow$ \textbf{1.14} &   {22.09} $\uparrow$\textbf{ 5.32} &   {24.17} $\downarrow$ 1.91 &   {16.93} $\uparrow$ \textbf{1.7} \\ \hline \hline
 & PGD-AT ~\cite{rice2020overfitting}       & 60.89          & 32.19          & 31.33          & 27.89          & 28.14          & 33.40          & 27.86          \\ %\cline{2-9} 
              & Trades~\cite{zhang2019theoretically}           & 58.61          & 29.20          & 28.44          & 25.95          & 26.21          & 29.81          & 25.94          \\ % \cline{2-9} 
              & AVmixup~\cite{lee2020adversarial}      & \underline{74.54}   &    38.89       &       \underline{33.55}         &      11.17          &       20.29         &       16.01         & 10.67          \\ \cline{2-9} 
          WideResNet34-10 & LAS-PGD-AT   &   {61.43} $\uparrow$ \textbf{0.54} &   {33.76} $\uparrow$ \textbf{1.57} &   {32.35} $\uparrow$ \textbf{1.02}&   \underline{29.08} $\uparrow$ \textbf{1.19}&   \underline{29.40} $\uparrow$ \textbf{1.26} &   \underline{34.49} $\uparrow$ \textbf{1.09} &   \underline{29.06} $\uparrow$ \textbf{1.2}\\ %\cline{2-9} 
                  & LAS-Trades  &   {60.74} $\uparrow$ \textbf{2.13} &   {31.65} $\uparrow$ \textbf{2.45} &   {30.69} $\uparrow$ \textbf{2.25} &   {27.10} $\uparrow$ \textbf{1.15} &   {27.41} $\uparrow$ \textbf{1.2}&   {31.59} $\uparrow$ \textbf{1.78} &   {27.10} $\uparrow$ \textbf{1.16} \\ %\cline{2-9} 
                  & LAS-AVmixup &       72.04 $\downarrow$ 2.5        &   \underline{41.93} $\uparrow$ \textbf{3.04}      &    24.23 $\downarrow$ 9.32         &      {17.09} $\uparrow$ \textbf{5.92}     & {25.36} $\uparrow$ \textbf{5.07}             &         {23.01}  $\uparrow$ \textbf{7.00 }       &       {16.15}         $\uparrow$ \textbf{5.48}   \\ \hline
\end{tabular}
}
 \vspace{-3mm}
\end{table*}

==> table/tb_cifar100_v4.tex <==
\begin{table*}[t]

\centering

\caption{ Comparisons on the CIFAR100 database. 
Numbers represent percentage. Number with underline indicates the best. 
%$\uparrow$ and $\downarrow$ indicate the performance change after the combination with our framework. 
% `a $\uparrow$ b' denotes that the accuracy is `a' and the improvement over the corresponding base model is `b'. `$\uparrow$' means `increase' and `$\downarrow$' means `decrease'. 
}
 \label{tb:cifar100}
 
 \vspace{-3mm}
 \scalebox{1}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
Target network                   & Method     & Clean          & PGD-10         & PGD-20         & PGD-50         & CW             & AA             \\ \hline \hline
\multirow{6}{*}{WideResNet34-10} & PGD-AT     & 60.89          & 32.19          & 31.69          & 31.45          & 30.1           & 27.86          \\ \cline{2-8} 
                                 & Trades     & 58.61          & 29.20          & 28.66          & 28.56          & 27.05          & 25.94          \\ \cline{2-8} 
                                 & AWP        & 60.38          & 34.13          & 33.86          & 33.65          & 31.12          & 28.86          \\ \cline{2-8} 
                                 & LAS-AT(ours)     & 61.80          & 33.45          & 32.77          & 32.54          & 31.12          & 29.03          \\ \cline{2-8} 
                                 & LAS-Trades(ours) & 60.62          & 32.99          & 32.53          & 32.39          & 29.51          & 28.12          \\ \cline{2-8} 
                                 & LAS-AWP(ours)    & \textbf{64.89} & \textbf{37.11} & \textbf{36.36} & \textbf{36.13} & \textbf{33.92} & \textbf{30.77} \\ \hline
\end{tabular}
}
 \vspace{-3mm}
\end{table*}

==> table/tb_cifar10_v2.tex <==
\begin{table*}[t]
\centering

\caption{ The comparison result on CIFAR10. }
 \label{table:table1}
 \scalebox{0.82}{
\begin{tabular}{c|c|cccccc|c}
\hline
Method        & Clean          & PGD-10         & APGD           & APGD-T         & FAB            & SQUARE         & AA             & Mean           \\ \hline \hline
Standard     & 94.72          & 0.0            & 1.80           & 1.40           & 63.00          & 64.70          & 0.0            & 21.82        \\ \hline\hline
SAT~\cite{madry2017towards}          & \textbf{84.50}  & 50.65          & 45.20          & 46.10          & 67.20          & 73.30          & 38.60          & 53.51          \\
RLAT-PGD     & 82.84 $\downarrow$  1.66   & \textbf{54.1} $\uparrow$ \textbf{3.45}  & \textbf{51.60} $\uparrow$ \textbf{6.40} & \textbf{52.10} $\uparrow$ \textbf{6.00} & \textbf{72.40}  $\uparrow$ \textbf{5.20} & \textbf{74.90}  $\uparrow$ \textbf{1.60}  & \textbf{42.40} $\uparrow$ \textbf{3.80}  & \textbf{57.92} $\uparrow$ \textbf{4.41} \\ \hline\hline
Trades~\cite{zhang2019theoretically}       & \textbf{82.20}          & 52.68          & 48.90          & 48.00          & 71.70          & \textbf{73.50}          & 39.82          & 55.77          \\
RLAT-Trades  & 80.97  $\downarrow$ 1.23         & \textbf{54.23} $\uparrow$ \textbf{1.55} & \textbf{51.90} $\uparrow$ \textbf{3.00} & \textbf{50.60} $\uparrow$ \textbf{2.60} & \textbf{71.80} $\uparrow$  & 72.90 $\downarrow$ 0.60 & \textbf{43.60} $\uparrow$  \textbf{3.78} & \textbf{57.51} $\uparrow$ \textbf{1.74} \\ \hline\hline
Avmixup~\cite{lee2020adversarial}      & 87.83          & 45.21          & 36.80          & 42.60          & 68.30          & 79.00          & 18.30          & 48.37          \\
RLAT-Avmixup & \textbf{90.71} $\uparrow$ \textbf{2.88} & \textbf{53.66} $\uparrow$ \textbf{8.45} & \textbf{58.40} $\uparrow$ \textbf{21.60} & \textbf{59.20} $\uparrow$ \textbf{16.60}   & \textbf{74.50} $\uparrow$ \textbf{6.20} & {79.00}  & \textbf{46.88}$\uparrow$  \textbf{28.58}& \textbf{61.94} $\uparrow$ \textbf{13.57}  \\ \hline
\end{tabular}
}
\end{table*}

==> table/tb_cifar10_v3.tex <==
\begin{table*}[t]

\centering

\caption{ Comparisons on the CIFAR10 database. 
Numbers represent percentage. Number with underline indicates the best. 
%$\uparrow$ and $\downarrow$ indicate the performance change after the combination with our framework. 
`a $\uparrow$ b' denotes that the accuracy is `a' and the improvement over the corresponding base model is `b'. `$\uparrow$' means `increase' and `$\downarrow$' means `decrease'.   
}
\label{tb:cifar10}

\vspace{-3mm}
 \scalebox{0.82}{
\begin{tabular}{c|c|cc|ccccc}
\hline
Target network  & Method       & Clean          & PGD-10         & APGD           & APGD-T         & FAB            & SQUARE         & AA             \\ \hline  \hline
   
        & PGD-AT~\cite{rice2020overfitting}     & 82.86         & 52.85          & 51.74          & 48.57          & 49.03          & 56.02          & 48.61          \\ %\cline{2-9} 
          & Trades~\cite{zhang2019theoretically}       & 82.02          & 53.08          & 51.49          & 48.92          & 49.37          & 55.06          & 48.87          \\ %\cline{2-9} 
          & AVmixup~\cite{lee2020adversarial}       & \underline{91.26}          & 60.19          & \underline{54.85}          & 19.19          & 37.14          & 36.20          & 19.19          \\ \cline{2-9} 
   {Resnet18}   & LAS-PGD-AT  & 82.05 $\downarrow$ 0.81   &  {54.23} $\uparrow$ \textbf{1.38} & {53.03} $\uparrow$ \textbf{1.29}  & \underline{50.08} $\uparrow$ \textbf{1.51}  &  {50.38} $\uparrow $ \textbf{1.35} &  \underline{56.13} $\uparrow$ \textbf{0.11} &  \underline{50.07} $\uparrow$ \textbf{1.46} \\ %\cline{2-9} 
      & LAS-Trades  & 81.97 $\downarrow$ 0.05  &  {54.09} $\uparrow$ \textbf{1.01} &  {52.88} $\uparrow$ \textbf{1.39}  &  {49.79} $\uparrow$ \textbf{0.87} &  {50.24} $\uparrow$ \textbf{0.87} &  {55.86} $\uparrow$ \textbf{0.80} &  {49.76} $\uparrow$ \textbf{0.89} \\ %\cline{2-9} 
      & LAS-AVmixup & 90.91 $\downarrow$ 0.35  &  \underline{63.00} $\uparrow$ \textbf{2.81} &  41.83 $\downarrow$ 13.02         &  {33.75} $\uparrow$ \textbf{14.56} &  \underline{51.16} $\uparrow$ \textbf{14.02} &  {45.77} $\uparrow$ \textbf{9.57} &  {33.47} $\uparrow$ \textbf{14.28} \\ \hline
    \hline
 & PGD-AT~\cite{rice2020overfitting}       & 85.17          & 56.07          & 54.56          & 51.71          & 52.25          & 59.12          & 51.66          \\ %\cline{2-9} 
      & Trades~\cite{zhang2019theoretically}        & 84.53          & 55.08          & 53.43          & 51.26          & 51.70          & 57.52          & 51.26          \\ %\cline{2-9} 
      & AVmixup~\cite{lee2020adversarial}         & \underline{94.44}          & 65.03          &   30.38             &     18.89           &    37.71            &        42.34        & 14.34          \\ \cline{2-9} 
      WideResNet34-10   & LAS-PGD-AT  &  {85.18} $\uparrow$ \textbf{0.01}  &  {57.65} $\uparrow$ \textbf{1.58} &  \underline{56.01} $\uparrow$ \textbf{1.45} &  \underline{53.78} $\uparrow$ \textbf{2.07} &  \underline{54.28} $\uparrow$ \textbf{2.03} &  \underline{59.80} $\uparrow$ \textbf{0.68} &  \underline{53.68} $\uparrow$ \textbf{2.02}\\ %\cline{2-9} 
          & LAS-Trades  &  {85.81} $\uparrow$ \textbf{1.28} &  {57.02} $\uparrow$ \textbf{1.94} &  {55.18} $\uparrow$ \textbf{1.75} &  {53.13} $\uparrow$ \textbf{1.87} &  {53.52} $\uparrow$ \textbf{1.82} &  {59.28} $\uparrow$ \textbf{1.76} &  {53.13} $\uparrow$ \textbf{1.87} \\ %\cline{2-9} 
              & LAS-AVmixup & 92.15 $\downarrow$ 2.29  &  \underline{69.89} $\uparrow$ \textbf{4.86}&          {34.91}   $\uparrow$ \textbf{4.53}     &   {24.41} $\uparrow$ \textbf{5.52}         &  {48.14} $\uparrow$\textbf{ 10.43} &  {48.21} $\uparrow$ \textbf{5.87} 
&         {24.40}  $\uparrow$ \textbf{10.06}      \\ \hline
\end{tabular}
}
\vspace{-3mm}
\end{table*}


% \begin{table*}[t]

% \centering

% \caption{ Comparisons with state-of-the-art methods on the CIFAR10 database. 
% Numbers in table represent percentage. Accuracy number in bold indicates the best. }
% \label{tb:cifar10}

% \vspace{2mm}
%  \scalebox{0.8}{
% \begin{tabular}{c|c|cc|ccccc}
% \hline
% Target network  & Method       & Clean          & PGD-10         & APGD           & APGD-T         & FAB            & SQUARE         & AA             \\ \hline  \hline
   
%         & PGD-AT~\cite{rice2020overfitting}     & 82.86         & 52.85          & 51.74          & 48.57          & 49.03          & 56.02          & 48.61          \\ %\cline{2-9} 
%           & Trades~\cite{zhang2019theoretically}       & 82.02          & 53.08          & 51.49          & 48.92          & 49.37          & 55.06          & 48.87          \\ %\cline{2-9} 
%           & AVmixup~\cite{lee2020adversarial}       & 91.26          & 60.19          & 54.85          & 19.19          & 37.14          & 36.20          & 19.19          \\ \cline{2-9} 
%   {Resnet18}                         & LAS-PGD-AT  & 82.05    &  {54.23} &  {53.03} &  {50.08} &  {50.38} &  {56.13} &  {50.07} \\ %\cline{2-9} 
%                           & LAS-Trades  & 81.97          &  {54.09} &  {52.88} &  {49.79} &  {50.24} &  {55.86} &  {49.76} \\ %\cline{2-9} 
%                           & LAS-AVmixup & 90.91          &  {63.00} & 41.83          &  {33.75} &  {51.16} &  {45.77} &  {33.47} \\ \hline
%                         \hline
%  & PGD-AT~\cite{rice2020overfitting}       & 85.17          & 56.07          & 54.56          & 51.71          & 52.25          & 59.12          & 51.66          \\ %\cline{2-9} 
%                           & Trades~\cite{zhang2019theoretically}        & 84.53          & 55.08          & 53.43          & 51.26          & 51.70          & 57.52          & 51.26          \\ %\cline{2-9} 
%                           & AVmixup~\cite{lee2020adversarial}         & 94.44          & 65.03          &   30.38             &     18.89           &    37.71            &        42.34        & 14.34          \\ \cline{2-9} 
%       WideResNet34-10                    & LAS-PGD-AT  &  {85.18} &  {57.65} &  {56.01} &  {53.78} &  {54.28} &  {59.80} &  {53.68} \\ %\cline{2-9} 
%                           & LAS-Trades  &  {85.81} &  {57.02} &  {55.18} &  {53.13} &  {53.52} &  {59.28} &  {53.13} \\ %\cline{2-9} 
%                               & LAS-AVmixup & 92.15          &  {69.89} &          {34.91}        &        {24.41}          &      {48.14}  &       {48.21}
%       &         {24.40}        \\ \hline
% \end{tabular}
% }
% \end{table*}

==> table/tb_cifar10_v4.tex <==
\begin{table*}[t]

\centering

\caption{ Comparisons on the CIFAR10 database. 
Numbers represent percentage. Number with underline indicates the best. 
%$\uparrow$ and $\downarrow$ indicate the performance change after the combination with our framework. 
% `a $\uparrow$ b' denotes that the accuracy is `a' and the improvement over the corresponding base model is `b'. `$\uparrow$' means `increase' and `$\downarrow$' means `decrease'.   
}
\label{tb:cifar10}

\vspace{-3mm}
 \scalebox{1}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
Target network                   & Method     & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W             & AA             \\ \hline \hline
\multirow{8}{*}{ResNet18}        & PGD-AT     & 82.56          & 52.85          & 52.27          & 51.98          & 50.89          & 48.54          \\ \cline{2-8} 
                                 & Trades     & 81.84          & 53.51          & 53.05          & 52.93          & 50.48          & 49.06          \\ \cline{2-8} 
                                 & FAT        & 87.97          & 47.58          & 47.35          & 46.98          & 49.92          & 43.90          \\ \cline{2-8} 
                                 & GAIRAT     & \textbf{83.22} & 55.78          & 55.23          & 54.81          & 39.86          & 33.35          \\ \cline{2-8} 
                                 & AWP        & 80.72          & 55.33          & 54.78          & 54.28          & 51.67          & 49.44          \\ \cline{2-8} 
                                 & LAS-AT(ours)     & 82.3           & 54.29          & 53.34          & 53.2           & 51.73          & 49.89          \\ \cline{2-8} 
                                 & LAS-Trades(ours) & 81.48          & 54.49          & 53.81          & 53.69          & 51.29          & 50.26          \\ \cline{2-8} 
                                 & LAS-AWP(ours)    & 83.03          & \textbf{56.45} & \textbf{55.76} & \textbf{55.43} & \textbf{53.06} & \textbf{50.77} \\ \hline \hline
\multirow{8}{*}{WideResNet34-10} & PGD-AT     & 85.17          & 56.07          & 55.08          & 54.88          & 53.91          & 51.69          \\ \cline{2-8} 
                                 & Trades     & 85.72          & 56.75          & 56.1           & 55.9           & 53.87          & 53.40          \\ \cline{2-8} 
                                 & FAT        & \textbf{89.65} & 50.01          & 49.49          & 48.79          & 48.50          & 47.48          \\ \cline{2-8} 
                                 & GAIRAT     & 86.30          & 60.64          & 59.54          & 58.74          & 45.57          & 40.30          \\ \cline{2-8} 
                                 & AWP        & 85.57          & 58.92          & 58.13          & 57.92          & 56.03          & 53.90          \\ \cline{2-8} 
                                 & LAS-AT(ours)     & 86.23          & 57.64          & 56.49          & 56.12          & 55.73          & 53.58          \\ \cline{2-8} 
                                 & LAS-Trades(ours) & 85.24          & 58.01          & 57.07          & 56.8           & 55.45          & 54.15          \\ \cline{2-8} 
                                 & LAS-AWP(ours)    & 87.74          & \textbf{61.09} & \textbf{60.16} & \textbf{59.79} & \textbf{58.22} & \textbf{55.52} \\ \hline
\end{tabular}
}
\vspace{-3mm}
\end{table*}


% \begin{table*}[t]

% \centering

% \caption{ Comparisons with state-of-the-art methods on the CIFAR10 database. 
% Numbers in table represent percentage. Accuracy number in bold indicates the best. }
% \label{tb:cifar10}

% \vspace{2mm}
%  \scalebox{0.8}{
% \begin{tabular}{c|c|cc|ccccc}
% \hline
% Target network  & Method       & Clean          & PGD-10         & APGD           & APGD-T         & FAB            & SQUARE         & AA             \\ \hline  \hline
   
%         & PGD-AT~\cite{rice2020overfitting}     & 82.86         & 52.85          & 51.74          & 48.57          & 49.03          & 56.02          & 48.61          \\ %\cline{2-9} 
%           & Trades~\cite{zhang2019theoretically}       & 82.02          & 53.08          & 51.49          & 48.92          & 49.37          & 55.06          & 48.87          \\ %\cline{2-9} 
%           & AVmixup~\cite{lee2020adversarial}       & 91.26          & 60.19          & 54.85          & 19.19          & 37.14          & 36.20          & 19.19          \\ \cline{2-9} 
%   {Resnet18}                         & LAS-PGD-AT  & 82.05    &  {54.23} &  {53.03} &  {50.08} &  {50.38} &  {56.13} &  {50.07} \\ %\cline{2-9} 
%                           & LAS-Trades  & 81.97          &  {54.09} &  {52.88} &  {49.79} &  {50.24} &  {55.86} &  {49.76} \\ %\cline{2-9} 
%                           & LAS-AVmixup & 90.91          &  {63.00} & 41.83          &  {33.75} &  {51.16} &  {45.77} &  {33.47} \\ \hline
%                         \hline
%  & PGD-AT~\cite{rice2020overfitting}       & 85.17          & 56.07          & 54.56          & 51.71          & 52.25          & 59.12          & 51.66          \\ %\cline{2-9} 
%                           & Trades~\cite{zhang2019theoretically}        & 84.53          & 55.08          & 53.43          & 51.26          & 51.70          & 57.52          & 51.26          \\ %\cline{2-9} 
%                           & AVmixup~\cite{lee2020adversarial}         & 94.44          & 65.03          &   30.38             &     18.89           &    37.71            &        42.34        & 14.34          \\ \cline{2-9} 
%       WideResNet34-10                    & LAS-PGD-AT  &  {85.18} &  {57.65} &  {56.01} &  {53.78} &  {54.28} &  {59.80} &  {53.68} \\ %\cline{2-9} 
%                           & LAS-Trades  &  {85.81} &  {57.02} &  {55.18} &  {53.13} &  {53.52} &  {59.28} &  {53.13} \\ %\cline{2-9} 
%                               & LAS-AVmixup & 92.15          &  {69.89} &          {34.91}        &        {24.41}          &      {48.14}  &       {48.21}
%       &         {24.40}        \\ \hline
% \end{tabular}
% }
% \end{table*}

==> table/tb_comparison_HP.tex <==
\begin{table*}[t]

\centering

\caption{ Comparisons with on advanced hyper-parameter methods on the CIFAR10 database. 
Numbers represent percentage. Number with underline indicates the best. 
%$\uparrow$ and $\downarrow$ indicate the performance change after the combination with our framework. 
% `a $\uparrow$ b' denotes that the accuracy is `a' and the improvement over the corresponding base model is `b'. `$\uparrow$' means `increase' and `$\downarrow$' means `decrease'. 
}
 \label{tb:cifar100}
 
 \vspace{-3mm}
 \scalebox{1}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
Target network                   & Method        & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W             & AA             \\ \hline \hline
\multirow{5}{*}{WideResNet34-10} & PGD-AT        & 85.17          & 56.07          & 55.08          & 54.88          & 53.91          & 51.69          \\ \cline{2-8} 
                                 & Random        & \textbf{88.05}          & 52.68          & 51.68          & 51.29          & 50.57          & 48.61          \\ \cline{2-8} 
                                 & OHP           & 86.34 & 56.67          & 55.35          & 54.94          & 54.47          & 52.22          \\ \cline{2-8} 
                                 & AdvHP         & 86.47          & 56.52          & 55.53          & 54.97          & 54.54          & 52.27          \\ \cline{2-8} 
                                 & LAS-AT(ours) & 86.23          & \textbf{57.64} & \textbf{56.49} & \textbf{56.12} & \textbf{55.73} & \textbf{53.58} \\ \hline
\end{tabular}
}
 \vspace{-3mm}
\end{table*}

==> table/tb_comparison_HP_v2.tex <==
\begin{table}[t]

\centering

\caption{ Comparisons with on advanced hyper-parameter methods on the CIFAR10 database. 
Numbers represent percentage. Number with underline indicates the best. 
%$\uparrow$ and $\downarrow$ indicate the performance change after the combination with our framework. 
% `a $\uparrow$ b' denotes that the accuracy is `a' and the improvement over the corresponding base model is `b'. `$\uparrow$' means `increase' and `$\downarrow$' means `decrease'. 
}
 \label{tb:comparsion_HP}
 
 \vspace{-3mm}
 \scalebox{0.9}{
\begin{tabular}{c|c|c|c|c}
\hline
Method       & Clean          & PGD-50         & C\&W           & AA             \\ \hline
PGD-AT~\cite{rice2020overfitting}       & 85.17          & 54.88          & 53.91          & 51.69          \\ \hline
Random       & \textbf{88.05} & 51.29          & 50.57          & 48.61          \\ \hline
OHL~\cite{lin2019online}        & 86.34          & 54.94          & 54.47          & 52.22          \\ \hline
AdvHP~\cite{DBLP:conf/iclr/ZhangWZZ20}        & 86.47          & 54.97          & 54.54          & 52.27          \\ \hline
LAS-AT(ours) & 86.23          & \textbf{56.12} & \textbf{55.73} & \textbf{53.58} \\ \hline
\end{tabular}
}
 \vspace{-3mm}
\end{table}

==> table/tb_tiny.tex <==
\begin{table}[t]
\centering

\caption{Results on the Tiny Imagenet database. Numbers in table represent percentage. $\uparrow$ and $\downarrow$ indicate performance change after plugging in our RLAT compared to the corresponding base model.  Number in bold indicate the best.}
\vspace{2mm}
 \label{tb:tiny}
\begin{tabular}{C{1.9cm}|C{1.2cm}|C{1.3cm} C{1.8cm}}
\hline
Method & Standard    & SAT~\cite{madry2017towards} & RLAT-SAT \\ \hline \hline
Clean  & {51.59} & {41.70} & \textbf{44.09} $\uparrow$ \textbf{2.39}  \\ \hline\hline
PGD-10 & 0.0  & 12.01 & \textbf{20.37} $\uparrow$ \textbf{8.36}  \\ 
APGD  & 3.0 & 12.40 & \textbf{21.20} $\uparrow$ \textbf{8.80}   \\ 
APGD-T & 2.70 & 13.60 & \textbf{18.10} $\uparrow$ \textbf{4.50}   \\ 
FAB    & 38.80 & 34.20 & \textbf{{36.20}} $\uparrow$ \textbf{2.00}  \\ 
SQUARE & 24.20 & 35.90 & \textbf{38.80} $\uparrow$ \textbf{2.90}  \\ 
AA     & 0.0 & 8.50 & \textbf{14.30} $\uparrow$ \textbf{5.80}  \\ \hline
Mean   & 11.45 & 22.62 & \textbf{27.58} $\uparrow$ \textbf{4.96}   \\ \hline
\end{tabular}
\end{table}

==> table/tb_tiny_v2.tex <==
\begin{table*}[t]
\centering
\footnotesize{
\caption{ THE COMPARISONS RESULT ON TINY IMAGENET. }
 \label{table:table3}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Model        & Clean          & PGD-10         & APGD           & APGD-T         & FAB            & SQUARE         & AA             & Mean           \\ \hline
Standard     & 51.59          & 0.0            & 3.00           & 2.70           & 38.80          & 24.20          & 0.0            & 17.18          \\ \hline
SAT          & 41.70          & 12.01          & 12.40          & 13.60          & 34.20          & 35.90          & 8.50           & 22.62          \\
RLAT-PGD     & \textbf{44.09} $\uparrow$  \textbf{2.39} & \textbf{20.37} $\uparrow$ \textbf{8.36} & \textbf{21.20} $\uparrow$  \textbf{8.80} & \textbf{18.10} $\uparrow$ \textbf{4.50} & \textbf{36.20} $\uparrow$  \textbf{2.00} & \textbf{38.80} $\uparrow$ \textbf{2.90} & \textbf{14.30} $\uparrow$ \textbf{5.80} & \textbf{27.58} $\uparrow$  \textbf{4.96} \\ \hline
Trades       & 33.17          & 12.03          & 14.90          & 16.30          & 28.50          & 30.50          & 7.60           & 20.42          \\
RLAT-Trades  & 0.0            & 0.0            & 0.0            & 0.0            & 0.0            & 0.0            & 0.0            & 0.0            \\ \hline
Avmixup      & 49.87          & 24.66          & 22.60          & 21.00          & 40.60          & 43.90          & 11.70          & 30.62          \\
RLAT-Avmixup & 0.0            & 0.0            & 0.0            & 0.0            & 0.0            & 0.0            & 0.0            & 0.0            \\ \hline
\end{tabular}
}
\end{table*}

==> table/tb_tiny_v3.tex <==
\begin{table*}[t]

\centering

\caption{ Comparisons on the Tiny Imagenet database. 
Numbers represent percentage. Number with underline indicates the best. 
%$\uparrow$ and $\downarrow$ indicate the performance change after the combination with our framework. 
`a $\uparrow$ b' denotes that the accuracy is `a' and the improvement over the corresponding base model is `b'. `$\uparrow$' means `increase' and `$\downarrow$' means `decrease'. 
}
 \label{tb:tiny}
 \vspace{-3mm}
\scalebox{0.82}{
\begin{tabular}{c|c|cc|ccccc}
\hline
Target network                 & Method      & Clean          & PGD-10         & APGD           & APGD-T         & FAB            & SQUARE         & AA             \\ \hline \hline
 & PGD-AT~\cite{rice2020overfitting}     & 43.98          & 20.34          & 15.94          & 13.82          & 13.86          & 19.94          & 13.78          \\ % \cline{2-9} 
         & Trades~\cite{zhang2019theoretically}      & 39.16          & 16.34          & 15.70          & 12.30          & 12.48          & 16.92          & 12.32          \\ %\cline{2-9} 
         & AVmixup~\cite{lee2020adversarial}     & \underline{49.46}          & {22.42}          & 20.84          & 6.74           & 7.94           & 18.30          & 5.42           \\ \cline{2-9} 
  PreActResNet18       & LAS-PGD-AT  &   {45.68} $\uparrow$ \textbf{1.70} &   {21.32} $\uparrow$ \textbf{0.98} &   {20.68} $\uparrow$ \textbf{4.74}&   \underline{{16.40}} $\uparrow$ \textbf{2.58} &   \underline{{16.54}} $\uparrow$ \textbf{2.68} &   {22.98} $\uparrow$ \textbf{3.04} &   \underline{{16.42}} $\uparrow$ \textbf{2.64} \\ % \cline{2-9} 
         & LAS-Trades  &   {43.20} $\uparrow$ \textbf{4.04} &   {18.82} $\uparrow$ \textbf{2.48} &   {18.44} $\uparrow$ \textbf{2.74} &   {13.48} $\uparrow$ \textbf{1.18} &   {13.72} $\uparrow$ \textbf{1.24} &   {20.02} $\uparrow$ \textbf{3.10} &   {13.50} $\uparrow$ \textbf{1.18}\\ %\cline{2-9} 
         & LAS-AVmixup & 47.54 $\downarrow$  1.92       &   \underline{{22.84}} $\uparrow$ \textbf{0.42} &   \underline{{22.10}} $\uparrow$ \textbf{1.26} &   {15.30} $\uparrow$ \textbf{8.56} &   {15.64} $\uparrow$ \textbf{7.70} &   \underline{{24.12}} $\uparrow$ \textbf{5.82}&   {15.30} $\uparrow$ \textbf{9.88} \\ \hline
\end{tabular}
}
 \vspace{-3mm}
\end{table*}

==> table/tb_tiny_v4.tex <==
\begin{table}[t]

\centering

\caption{ Comparisons on the Tiny Imagenet database. 
Numbers represent percentage. Number with underline indicates the best. 
%$\uparrow$ and $\downarrow$ indicate the performance change after the combination with our framework. 
% `a $\uparrow$ b' denotes that the accuracy is `a' and the improvement over the corresponding base model is `b'. `$\uparrow$' means `increase' and `$\downarrow$' means `decrease'. 
}
 \label{tb:tiny}
 \vspace{-3mm}
\scalebox{0.9}{
\begin{tabular}{|c|c|c|c}
\hline
Target network                  & Method     & Clean          & PGD-50         & AA             \\ \hline \hline
\multirow{6}{*}{PreActResNet18} & PGD-AT     & 43.98          & 20.34          & 13.78          \\ \cline{2-5} 
                                & Trades     & 39.16          & 16.34          & 12.32          \\ \cline{2-5} 
                                & AWP        & 41.48          & 22.51          & 17.34          \\ \cline{2-5} 
                                & LAS-AT     & 44.86          & 22.16          & 16.74          \\ \cline{2-5} 
                                & LAS-Trades & 41.38          & 18.36          & 14.08          \\ \cline{2-5} 
                                & LAS-AWP    & \textbf{45.26} & \textbf{23.42} & \textbf{18.42} \\ \hline
\end{tabular}
}
 \vspace{-3mm}
\end{table}
